Pure Interchange Oscillations of Thin Filaments in an Average Magnetosphere

This paper describes magnetospheric waves of very long wavelength in thin magnetic filaments. We consider an average magnetospheric configuration with zero ionospheric conductance and calculate waves using two different formulations: classic interchange theory and ideal MHD. Classic interchange theory, which is developed in detail in this paper, is basically analytic and is relatively straightforward to determine computationally, but it cannot offer very high accuracy. The two formalisms agree well for the plasma sheet and also for the inner magnetosphere. The eigenfrequencies range over about a factor of seven, but the formulations generally agree with a root-mean-square difference between the logarithms of interchange and MHD frequencies to be $\sim 0.054$. The pressure perturbations in the classic interchange theory are assumed constant along each field line, but the MHD computed pressure perturbations along the field line vary in a range $\sim 30 \%$ in the plasma sheet but are larger in the inner magnetosphere. The parallel and perpendicular displacements, which are very different in the plasma sheet and inner magnetosphere, show good qualitative agreement between the two approaches. In the plasma sheet, the perpendicular displacements are strongly concentrated in the equatorial plane, whereas the parallel displacements are spread through most of the plasma sheet away from the equatorial plane; and can be regarded as buoyancy waves. In the inner magnetosphere, the displacements are more sinusoidal and are more like conventional slow modes. The different forms of the waves are best characterized by the flux tube entropy $PV^\gamma$.

==> Pure Interchange Oscillations of Thin Filaments/trackchanges-0.7.0/README <==

TrackChanges
Multiple editors in LaTeX.
========================================================================

INTRODUCTION:

  The TrackChanges package consists of two parts:
  1.  A LaTex style file: 
        trackchanges.sty
  2.  A GUI, written in python:
         trackchanges.py

  The style file may be used without the GUI.  The GUI is to be used to
  facilitate accepting, rejecting, or modifying the edits made using the
  commands defined in the style file.

  This packages also includes a command line utility: acceptchanges.py.
  This utility will only work in posix environments.

  Help files are available as part of this package:
    ./documentation/web/help.html

  Documentation is also  available at the TrackChanges website.

  To get the latest version of this sofware go to:
    http://trackchanges.sourceforge.net

========================================================================

LaTeX STYLEFILE:

  INSTALLATION:
    Copy the style file to the directory with your LaTeX document.
    The style file can be found at: ./LatexPackage/trackchanges.sty

  USAGE:
    Add the following line to you latex document:
      \usepackage{trackchanges}

    Add the names of the editors in the preamble [OPTIONAL]:
      \addeditor{editor}

    Now you have access to all of the TrackChanges commands:
      \add[editor]{added text}
      \remove[editor]{removed text}
      \change[editor]{removed text}{added text}
      \note[editor]{note text}
      \annote[editor]{text to annotate}{note text}

    See the documentation or website for display options.

========================================================================

TRACKCHANGES GUI

  This is a Beta version of the TrackChanges GUI. 
  That means: Beware! Bugs may lurk ahead.

  If you choose to use this software plese be careful to back up your 
  TeX files.  This software has not been thoroughly tested and may
  corrupt your TeX files.  (The style file is fine and can't mess any
  thing up but the GUI for accepting/rejecting/modifying might.)

  ----------------------------------------------------------------------
  
  WARNING:  
    This program has not be generalized to handle international
    characters.  Such characters may cause unexpected behavior.
  
  NOTE:
    So far the GUI has only been tested on Windows XP and Os X.
    While it should work on linux, it might not.
  
  WARNING (AGAIN):
    This is beta software. It has not been tested much.
    Things may be broken.
  
  
  
  ----------------------------------------------------------------------
  INSTALLATION:
    Once you have all the dependencies installed, 
    just run ./PythonPackage/trackchanges.py
    
      $> cd PythonPackage
      $> python trackchanges.py
  
  
  ----------------------------------------------------------------------
  DEPENDANCIES:
    To get the trackchanges GUI to run you will need several things:
     
    1. Python 2.6 or later
    2. PyQt 4.4.4 or later
  
  ----------------------------------------------------------------------
  WHERE TO GET DEPENDANCIES:
    Python 2.6  -- http://www.python.org/
    PyQt 4      -- http://www.riverbankcomputing.co.uk/
  
  


========================================================================

This file is part of TrackChanges
Copyright 2009 Novimir Antoniuk Pablant
               Felix Salfner

TrackChanges is free software: you can redistribute it and/or modify
it under the terms of the GNU General Public License as published by
the Free Software Foundation, either version 2 of the License, or
(at your option) any later version.

TrackChanges is distributed in the hope that it will be useful,
but WITHOUT ANY WARRANTY; without even the implied warranty of
MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
GNU General Public License for more details.

You should have received a copy of the GNU General Public License
along with TrackChanges.  If not, see <http://www.gnu.org/licenses/>.

------------------------------------------------------------------------

==> trackchanges-0.7.0/README <==

TrackChanges
Multiple editors in LaTeX.
========================================================================

INTRODUCTION:

  The TrackChanges package consists of two parts:
  1.  A LaTex style file: 
        trackchanges.sty
  2.  A GUI, written in python:
         trackchanges.py

  The style file may be used without the GUI.  The GUI is to be used to
  facilitate accepting, rejecting, or modifying the edits made using the
  commands defined in the style file.

  This packages also includes a command line utility: acceptchanges.py.
  This utility will only work in posix environments.

  Help files are available as part of this package:
    ./documentation/web/help.html

  Documentation is also  available at the TrackChanges website.

  To get the latest version of this sofware go to:
    http://trackchanges.sourceforge.net

========================================================================

LaTeX STYLEFILE:

  INSTALLATION:
    Copy the style file to the directory with your LaTeX document.
    The style file can be found at: ./LatexPackage/trackchanges.sty

  USAGE:
    Add the following line to you latex document:
      \usepackage{trackchanges}

    Add the names of the editors in the preamble [OPTIONAL]:
      \addeditor{editor}

    Now you have access to all of the TrackChanges commands:
      \add[editor]{added text}
      \remove[editor]{removed text}
      \change[editor]{removed text}{added text}
      \note[editor]{note text}
      \annote[editor]{text to annotate}{note text}

    See the documentation or website for display options.

========================================================================

TRACKCHANGES GUI

  This is a Beta version of the TrackChanges GUI. 
  That means: Beware! Bugs may lurk ahead.

  If you choose to use this software plese be careful to back up your 
  TeX files.  This software has not been thoroughly tested and may
  corrupt your TeX files.  (The style file is fine and can't mess any
  thing up but the GUI for accepting/rejecting/modifying might.)

  ----------------------------------------------------------------------
  
  WARNING:  
    This program has not be generalized to handle international
    characters.  Such characters may cause unexpected behavior.
  
  NOTE:
    So far the GUI has only been tested on Windows XP and Os X.
    While it should work on linux, it might not.
  
  WARNING (AGAIN):
    This is beta software. It has not been tested much.
    Things may be broken.
  
  
  
  ----------------------------------------------------------------------
  INSTALLATION:
    Once you have all the dependencies installed, 
    just run ./PythonPackage/trackchanges.py
    
      $> cd PythonPackage
      $> python trackchanges.py
  
  
  ----------------------------------------------------------------------
  DEPENDANCIES:
    To get the trackchanges GUI to run you will need several things:
     
    1. Python 2.6 or later
    2. PyQt 4.4.4 or later
  
  ----------------------------------------------------------------------
  WHERE TO GET DEPENDANCIES:
    Python 2.6  -- http://www.python.org/
    PyQt 4      -- http://www.riverbankcomputing.co.uk/
  
  


========================================================================

This file is part of TrackChanges
Copyright 2009 Novimir Antoniuk Pablant
               Felix Salfner

TrackChanges is free software: you can redistribute it and/or modify
it under the terms of the GNU General Public License as published by
the Free Software Foundation, either version 2 of the License, or
(at your option) any later version.

TrackChanges is distributed in the hope that it will be useful,
but WITHOUT ANY WARRANTY; without even the implied warranty of
MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
GNU General Public License for more details.

You should have received a copy of the GNU General Public License
along with TrackChanges.  If not, see <http://www.gnu.org/licenses/>.

------------------------------------------------------------------------
